Galaxies in voids assemble their stars slowly

Galaxies in the Universe are distributed in a web-like structure characterised by different large-scale environments: dense clusters, elongated filaments, sheetlike walls, and under-dense regions, called voids. The low density in voids is expected to affect the properties of their galaxies. Indeed, previous studies have shown that galaxies in voids are on average bluer and less massive, and have later morphologies and higher current star formation rates than galaxies in denser large-scale environments. However, it has never been observationally proved that the star formation histories (SFHs) in void galaxies are substantially different from those in filaments, walls, and clusters. Here we show that void galaxies have had, on average, slower SFHs than galaxies in denser large-scale environments. We also find two main SFH types present in all the environments: 'short-timescale' galaxies are not affected by their large-scale environment at early times but only later in their lives; 'long-timescale' galaxies have been continuously affected by their environment and stellar mass. Both types have evolved slower in voids than in filaments, walls, and clusters.

==> bib_macro.tex <==
\newcommand*\aap{Astron. Astrophys.}
\let\astap=\aap
\newcommand*\aapr{A\&A~Rev.}
\newcommand*\aaps{A\&AS}
\newcommand*\actaa{Acta Astron.}
\newcommand*\aj{Astron. J.}
\newcommand*\ao{Appl.~Opt.}
\let\applopt\ao
\newcommand*\apj{Astrophys. J.}
\newcommand*\apjl{Astrophys. J.}
\let\apjlett\apjl
\newcommand*\apjs{ApJS}
\let\apjsupp\apjs
\newcommand*\aplett{Astrophys.~Lett.}
\newcommand*\apspr{Astrophys.~Space~Phys.~Res.}
\newcommand*\apss{Ap\&SS}
\newcommand*\araa{ARA\&A}
\newcommand*\azh{AZh}
\newcommand*\baas{BAAS}
\newcommand*\bac{Bull. astr. Inst. Czechosl.}
\newcommand*\bain{Bull.~Astron.~Inst.~Netherlands}
\newcommand*\caa{Chinese Astron. Astrophys.}
\newcommand*\cjaa{Chinese J. Astron. Astrophys.}
\newcommand*\fcp{Fund.~Cosmic~Phys.}
\newcommand*\gca{Geochim.~Cosmochim.~Acta}
\newcommand*\grl{Geophys.~Res.~Lett.}
\newcommand*\iaucirc{IAU~Circ.}
\newcommand*\icarus{Icarus}
\newcommand*\jcap{J. Cosmology Astropart. Phys.}
\newcommand*\jcp{J.~Chem.~Phys.}
\newcommand*\jgr{J.~Geophys.~Res.}
\newcommand*\jqsrt{J.~Quant.~Spectr.~Rad.~Transf.}
\newcommand*\jrasc{JRASC}
\newcommand*\memras{MmRAS}
\newcommand*\memsai{Mem.~Soc.~Astron.~Italiana}
\newcommand*\mnras{Mon. Not. R. Astron. Soc.}
\newcommand*\na{New A}
\newcommand*\nar{New A Rev.}
\newcommand*\nat{Nature}
\newcommand*\nphysa{Nucl.~Phys.~A}
\newcommand*\pasa{PASA}
\newcommand*\pasj{PASJ}
\newcommand*\pasp{PASP}
\newcommand*\physrep{Phys.~Rep.}
\newcommand*\physscr{Phys.~Scr}
\newcommand*\planss{Planet.~Space~Sci.}
\newcommand*\pra{Phys.~Rev.~A}
\newcommand*\prb{Phys.~Rev.~B}
\newcommand*\prc{Phys.~Rev.~C}
\newcommand*\prd{Phys.~Rev.~D}
\newcommand*\pre{Phys.~Rev.~E}
\newcommand*\prl{Phys.~Rev.~Lett.}
\newcommand*\procspie{Proc.~SPIE}
\newcommand*\qjras{QJRAS}
\newcommand*\rmxaa{Rev. Mexicana Astron. Astrofis.}
\newcommand*\skytel{S\&T}
\newcommand*\solphys{Sol.~Phys.}
\newcommand*\sovast{Soviet~Ast.}
\newcommand*\ssr{Space~Sci.~Rev.}
\newcommand*\zap{ZAp}

==> main_bib.tex <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{16}
% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\url{https://doi.org/#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\bibcommenthead
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

%%% 1
\bibitem{2001ApJ...557..495P}
\begin{barticle}
\bauthor{\bsnm{{Peebles}}, \binits{P.J.E.}}:
\batitle{{The Void Phenomenon}}.
\bjtitle{\apj}
\bvolume{557}(\bissue{2}),
\bfpage{495}--\blpage{504}
(\byear{2001})
%{\href{https://arxiv.org/abs/astro-ph/0101127}{{arXiv:astro-ph/0101127}}}
%{[astro-ph]}.
%\doiurl{10.1086/322254}
\end{barticle}
\endbibitem

%%% 2
\bibitem{2011AJ....141....4K}
\begin{barticle}
\bauthor{\bsnm{{Kreckel}}, \binits{K.}},
\bauthor{et al.}:
%\bauthor{\bsnm{{Platen}}, \binits{E.}},
%\bauthor{\bsnm{{Arag{\'o}n-Calvo}}, \binits{M.A.}},
%\bauthor{\bsnm{{van Gorkom}}, \binits{J.H.}},
%\bauthor{\bsnm{{van de Weygaert}}, \binits{R.}},
%\bauthor{\bsnm{{van der Hulst}}, \binits{J.M.}},
%\bauthor{\bsnm{{Kova{\v{c}}}}, \binits{K.}},
%\bauthor{\bsnm{{Yip}}, \binits{C.-W.}},
%\bauthor{\bsnm{{Peebles}}, \binits{P.J.E.}}:
\batitle{{Only the Lonely: H I Imaging of Void Galaxies}}.
\bjtitle{\aj}
\bvolume{141}(\bissue{1}),
\bfpage{4}
(\byear{2011})
%{\href{https://arxiv.org/abs/1008.4616}{{arXiv:1008.4616}}}
%{[astro-ph.CO]}.
%\doiurl{10.1088/0004-6256/141/1/4}
\end{barticle}
\endbibitem

%%% 3
\bibitem{2012MNRAS.421..926P}
\begin{barticle}
\bauthor{\bsnm{{Pan}}, \binits{D.C.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
\bauthor{\bsnm{{Hoyle}}, \binits{F.}},
\bauthor{\bsnm{{Choi}}, \binits{Y.-Y.}},
\bauthor{\bsnm{{Park}}, \binits{C.}}:
\batitle{{Cosmic voids in Sloan Digital Sky Survey Data Release 7}}.
\bjtitle{\mnras}
\bvolume{421}(\bissue{2}),
\bfpage{926}--\blpage{934}
(\byear{2012})
%{\href{https://arxiv.org/abs/1103.4156}{{arXiv:1103.4156}}}
%{[astro-ph.CO]}.
%\doiurl{10.1111/j.1365-2966.2011.20197.x}
\end{barticle}
\endbibitem

%%% 4
\bibitem{2012ApJ...744...82V}
\begin{barticle}
\bauthor{\bsnm{{Varela}}, \binits{J.}},
\bauthor{\bsnm{{Betancort-Rijo}}, \binits{J.}},
\bauthor{\bsnm{{Trujillo}}, \binits{I.}},
\bauthor{\bsnm{{Ricciardelli}}, \binits{E.}}:
\batitle{{The Orientation of Disk Galaxies around Large Cosmic Voids}}.
\bjtitle{\apj}
\bvolume{744}(\bissue{2}),
\bfpage{82}
(\byear{2012})
%{\href{https://arxiv.org/abs/1109.2056}{{arXiv:1109.2056}}}
%{[astro-ph.CO]}.
%\doiurl{10.1088/0004-637X/744/2/82}
\end{barticle}
\endbibitem

%%% 5
\bibitem{2016IAUS..308..493V}
\begin{bchapter}
\bauthor{\bsnm{{van de Weygaert}}, \binits{R.}}:
\bctitle{{Voids and the Cosmic Web: cosmic depression \& spatial complexity}}.
In: \beditor{\bsnm{{van de Weygaert}}, \binits{R.}},
\beditor{\bsnm{{Shandarin}}, \binits{S.}},
\beditor{\bsnm{{Saar}}, \binits{E.}},
\beditor{\bsnm{{Einasto}}, \binits{J.}} (eds.)
\bbtitle{The Zeldovich Universe: Genesis and Growth of the Cosmic Web},
vol. \bseriesno{308},
pp. \bfpage{493}--\blpage{523}
(\byear{2016}).
%\doiurl{10.1017/S1743921316010504}
\end{bchapter}
\endbibitem

%%% 6
\bibitem{2004ApJ...617...50R}
\begin{barticle}
\bauthor{\bsnm{{Rojas}}, \binits{R.R.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
\bauthor{\bsnm{{Hoyle}}, \binits{F.}},
\bauthor{\bsnm{{Brinkmann}}, \binits{J.}}:
\batitle{{Photometric Properties of Void Galaxies in the Sloan Digital Sky
  Survey}}.
\bjtitle{\apj}
\bvolume{617}(\bissue{1}),
\bfpage{50}--\blpage{63}
(\byear{2004})
%{\href{https://arxiv.org/abs/astro-ph/0307274}{{arXiv:astro-ph/0307274}}}
%{[astro-ph]}.
%\doiurl{10.1086/425225}
\end{barticle}
\endbibitem

%%% 7
\bibitem{2005ApJ...624..571R}
\begin{barticle}
\bauthor{\bsnm{{Rojas}}, \binits{R.R.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
\bauthor{\bsnm{{Hoyle}}, \binits{F.}},
\bauthor{\bsnm{{Brinkmann}}, \binits{J.}}:
\batitle{{Spectroscopic Properties of Void Galaxies in the Sloan Digital Sky
  Survey}}.
\bjtitle{\apj}
\bvolume{624}(\bissue{2}),
\bfpage{571}--\blpage{585}
(\byear{2005})
%{\href{https://arxiv.org/abs/astro-ph/0409074}{{arXiv:astro-ph/0409074}}}
%{[astro-ph]}.
%\doiurl{10.1086/428476}
\end{barticle}
\endbibitem

%%% 8
\bibitem{2006MNRAS.372.1710P}
\begin{barticle}
\bauthor{\bsnm{{Patiri}}, \binits{S.G.}},
\bauthor{\bsnm{{Prada}}, \binits{F.}},
\bauthor{\bsnm{{Holtzman}}, \binits{J.}},
\bauthor{\bsnm{{Klypin}}, \binits{A.}},
\bauthor{\bsnm{{Betancort-Rijo}}, \binits{J.}}:
\batitle{{The properties of galaxies in voids}}.
\bjtitle{\mnras}
\bvolume{372}(\bissue{4}),
\bfpage{1710}--\blpage{1720}
(\byear{2006})
%{\href{https://arxiv.org/abs/astro-ph/0605703}{{arXiv:astro-ph/0605703}}}
%{[astro-ph]}.
%\doiurl{10.1111/j.1365-2966.2006.10975.x}
\end{barticle}
\endbibitem

%%% 9
\bibitem{2007ApJ...658..898P}
\begin{barticle}
\bauthor{\bsnm{{Park}}, \binits{C.}},
\bauthor{et al.}:
%\bauthor{\bsnm{{Choi}}, \binits{Y.-Y.}},
%\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
%\bauthor{\bsnm{{Gott}}, \binits{I.} \bsuffix{J.~Richard}},
%\bauthor{\bsnm{{Blanton}}, \binits{M.R.}},
%\bauthor{\bsnm{{SDSS Collaboration}}}:
\batitle{{Environmental Dependence of Properties of Galaxies in the Sloan Digital Sky Survey}}.
\bjtitle{\apj}
\bvolume{658}(\bissue{2}),
\bfpage{898}--\blpage{916}
(\byear{2007})
%{\href{https://arxiv.org/abs/astro-ph/0611610}{{arXiv:astro-ph/0611610}}}
%{[astro-ph]}.
%\doiurl{10.1086/511059}
\end{barticle}
\endbibitem

%%% 10
\bibitem{2012MNRAS.426.3041H}
\begin{barticle}
\bauthor{\bsnm{{Hoyle}}, \binits{F.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
\bauthor{\bsnm{{Pan}}, \binits{D.}}:
\batitle{{Photometric properties of void galaxies in the Sloan Digital Sky
  Survey Data Release 7}}.
\bjtitle{\mnras}
\bvolume{426}(\bissue{4}),
\bfpage{3041}--\blpage{3050}
(\byear{2012})
%{\href{https://arxiv.org/abs/1205.1843}{{arXiv:1205.1843}}}
%{[astro-ph.CO]}.
%\doiurl{10.1111/j.1365-2966.2012.21943.x}
\end{barticle}
\endbibitem

%%% 11
\bibitem{2012AJ....144...16K}
\begin{barticle}
\bauthor{\bsnm{{Kreckel}}, \binits{K.}},
\bauthor{et al.}:
%\bauthor{\bsnm{{Platen}}, \binits{E.}},
%\bauthor{\bsnm{{Arag{\'o}n-Calvo}}, \binits{M.A.}},
%\bauthor{\bsnm{{van Gorkom}}, \binits{J.H.}},
%\bauthor{\bsnm{{van de Weygaert}}, \binits{R.}},
%\bauthor{\bsnm{{van der Hulst}}, \binits{J.M.}},
%\bauthor{\bsnm{{Beygu}}, \binits{B.}}:
\batitle{{The Void Galaxy Survey: Optical Properties and H I Morphology and
  Kinematics}}.
\bjtitle{\aj}
\bvolume{144}(\bissue{1}),
\bfpage{16}
(\byear{2012})
%{\href{https://arxiv.org/abs/1204.5185}{{arXiv:1204.5185}}}
%{[astro-ph.CO]}.
%\doiurl{10.1088/0004-6256/144/1/16}
\end{barticle}
\endbibitem

%%% 12
\bibitem{2014MNRAS.445.4045R}
\begin{barticle}
\bauthor{\bsnm{{Ricciardelli}}, \binits{E.}},
\bauthor{\bsnm{{Cava}}, \binits{A.}},
\bauthor{\bsnm{{Varela}}, \binits{J.}},
\bauthor{\bsnm{{Quilis}}, \binits{V.}}:
\batitle{{The star formation activity in cosmic voids}}.
\bjtitle{\mnras}
\bvolume{445}(\bissue{4}),
\bfpage{4045}--\blpage{4054}
(\byear{2014})
%{\href{https://arxiv.org/abs/1410.0023}{{arXiv:1410.0023}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stu2061}
\end{barticle}
\endbibitem

%%% 13
\bibitem{2016MNRAS.458..394B}
\begin{barticle}
\bauthor{\bsnm{{Beygu}}, \binits{B.}},
\bauthor{et al.}:
%\bauthor{\bsnm{{Kreckel}}, \binits{K.}},
%\bauthor{\bsnm{{van der Hulst}}, \binits{J.M.}},
%\bauthor{\bsnm{{Jarrett}}, \binits{T.H.}},
%\bauthor{\bsnm{{Peletier}}, \binits{R.}},
%\bauthor{\bsnm{{van de Weygaert}}, \binits{R.}},
%\bauthor{\bsnm{{van Gorkom}}, \binits{J.H.}},
%\bauthor{\bsnm{{Aragon-Calvo}}, \binits{M.A.}}:
\batitle{{The void galaxy survey: Star formation properties}}.
\bjtitle{\mnras}
\bvolume{458}(\bissue{1}),
\bfpage{394}--\blpage{409}
(\byear{2016})
%{\href{https://arxiv.org/abs/1601.08228}{{arXiv:1601.08228}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stw280}
\end{barticle}
\endbibitem

%%% 14
\bibitem{2021ApJ...906...97F}
\begin{barticle}
\bauthor{\bsnm{{Florez}}, \binits{J.}},
\bauthor{et al.}:
%\bauthor{\bsnm{{Berlind}}, \binits{A.A.}},
%\bauthor{\bsnm{{Kannappan}}, \binits{S.J.}},
%\bauthor{\bsnm{{Stark}}, \binits{D.V.}},
%\bauthor{\bsnm{{Eckert}}, \binits{K.D.}},
%\bauthor{\bsnm{{Calderon}}, \binits{V.F.}},
%\bauthor{\bsnm{{Moffett}}, \binits{A.J.}},
%\bauthor{\bsnm{{Campbell}}, \binits{D.}},
%\bauthor{\bsnm{{Sinha}}, \binits{M.}}:
\batitle{{Void Galaxies Follow a Distinct Evolutionary Path in the
  Environmental COntext Catalog}}.
\bjtitle{\apj}
\bvolume{906}(\bissue{2}),
\bfpage{97}
(\byear{2021})
%{\href{https://arxiv.org/abs/2011.08276}{{arXiv:2011.08276}}}
%{[astro-ph.GA]}.
%\doiurl{10.3847/1538-4357/abca9f}
\end{barticle}
\endbibitem

%%% 15
\bibitem{1996AJ....111.2150S}
\begin{barticle}
\bauthor{\bsnm{{Szomoru}}, \binits{A.}},
\bauthor{\bsnm{{van Gorkom}}, \binits{J.H.}},
\bauthor{\bsnm{{Gregg}}, \binits{M.D.}},
\bauthor{\bsnm{{Strauss}}, \binits{M.A.}}:
\batitle{{An HI Survey of the Bootes Void. II. The Analysis}}.
\bjtitle{\aj}
\bvolume{111},
\bfpage{2150}
(\byear{1996})
%{\href{https://arxiv.org/abs/astro-ph/9511128}{{arXiv:astro-ph/9511128}}}
%{[astro-ph]}.
%\doiurl{10.1086/117951}
\end{barticle}
\endbibitem

%%% 16
\bibitem{2013AJ....145..120B}
\begin{barticle}
\bauthor{\bsnm{{Beygu}}, \binits{B.}},
\bauthor{\bsnm{{Kreckel}}, \binits{K.}},
\bauthor{\bsnm{{van de Weygaert}}, \binits{R.}},
\bauthor{\bsnm{{van der Hulst}}, \binits{J.M.}},
\bauthor{\bsnm{{van Gorkom}}, \binits{J.H.}}:
\batitle{{An Interacting Galaxy System along a Filament in a Void}}.
\bjtitle{\aj}
\bvolume{145}(\bissue{5}),
\bfpage{120}
(\byear{2013})
%{\href{https://arxiv.org/abs/1303.0538}{{arXiv:1303.0538}}}
%{[astro-ph.CO]}.
%\doiurl{10.1088/0004-6256/145/5/120}
\end{barticle}
\endbibitem

\end{thebibliography}


==> methods_bib.tex <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{99}

% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\url{https://doi.org/#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\bibcommenthead
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

\newcounter{mycounterbib}
\setcounter{mycounterbib}{16}
%\addtocounter{enumi}{16}

%\let\myvalue\thenumi
%%% 17
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{CAVITYweb}
\begin{botherref}
Calar Alto Void Integral-field Treasury surveY.
\url{https://cavity.caha.es/}
\end{botherref}
\endbibitem

%%% 18
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{CAHAweb}
\begin{botherref}
Calar Alto Observatory.
\url{https://www.caha.es/}
\end{botherref}
\endbibitem

%%% 19
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{1997ApJ...491..421E}
\begin{barticle}
\bauthor{\bsnm{{El-Ad}}, \binits{H.}},
\bauthor{\bsnm{{Piran}}, \binits{T.}}:
\batitle{{Voids in the Large-Scale Structure}}.
\bjtitle{\apj}
\bvolume{491}(\bissue{2}),
\bfpage{421}--\blpage{435}
(\byear{1997})
%{\href{https://arxiv.org/abs/astro-ph/9702135}{{arXiv:astro-ph/9702135}}}
%{[astro-ph]}.
%\doiurl{10.1086/304973}
\end{barticle}
\endbibitem

%%% 20
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2002ApJ...566..641H}
\begin{barticle}
\bauthor{\bsnm{{Hoyle}}, \binits{F.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}}:
\batitle{{Voids in the Point Source Catalogue Survey and the Updated Zwicky
  Catalog}}.
\bjtitle{\apj}
\bvolume{566}(\bissue{2}),
\bfpage{641}--\blpage{651}
(\byear{2002})
%{\href{https://arxiv.org/abs/astro-ph/0109357}{{arXiv:astro-ph/0109357}}}
%{[astro-ph]}.
%\doiurl{10.1086/338340}
\end{barticle}
\endbibitem

%%% 21
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2009ApJS..182..543A}
\begin{barticle}
\bauthor{\bsnm{{Abazajian}}, \binits{K.N.}},
\begin{comment}
\bauthor{\bsnm{{Adelman-McCarthy}}, \binits{J.K.}},
\bauthor{\bsnm{{Ag{\"u}eros}}, \binits{M.A.}},
\bauthor{\bsnm{{Allam}}, \binits{S.S.}},
\bauthor{\bsnm{{Allende Prieto}}, \binits{C.}},
\bauthor{\bsnm{{An}}, \binits{D.}},
\bauthor{\bsnm{{Anderson}}, \binits{K.S.J.}},
\bauthor{\bsnm{{Anderson}}, \binits{S.F.}},
\bauthor{\bsnm{{Annis}}, \binits{J.}},
\bauthor{\bsnm{{Bahcall}}, \binits{N.A.}},
\bauthor{\bsnm{{Bailer-Jones}}, \binits{C.A.L.}},
\bauthor{\bsnm{{Barentine}}, \binits{J.C.}},
\bauthor{\bsnm{{Bassett}}, \binits{B.A.}},
\bauthor{\bsnm{{Becker}}, \binits{A.C.}},
\bauthor{\bsnm{{Beers}}, \binits{T.C.}},
\bauthor{\bsnm{{Bell}}, \binits{E.F.}},
\bauthor{\bsnm{{Belokurov}}, \binits{V.}},
\bauthor{\bsnm{{Berlind}}, \binits{A.A.}},
\bauthor{\bsnm{{Berman}}, \binits{E.F.}},
\bauthor{\bsnm{{Bernardi}}, \binits{M.}},
\bauthor{\bsnm{{Bickerton}}, \binits{S.J.}},
\bauthor{\bsnm{{Bizyaev}}, \binits{D.}},
\bauthor{\bsnm{{Blakeslee}}, \binits{J.P.}},
\bauthor{\bsnm{{Blanton}}, \binits{M.R.}},
\bauthor{\bsnm{{Bochanski}}, \binits{J.J.}},
\bauthor{\bsnm{{Boroski}}, \binits{W.N.}},
\bauthor{\bsnm{{Brewington}}, \binits{H.J.}},
\bauthor{\bsnm{{Brinchmann}}, \binits{J.}},
\bauthor{\bsnm{{Brinkmann}}, \binits{J.}},
\bauthor{\bsnm{{Brunner}}, \binits{R.J.}},
\bauthor{\bsnm{{Budav{\'a}ri}}, \binits{T.}},
\bauthor{\bsnm{{Carey}}, \binits{L.N.}},
\bauthor{\bsnm{{Carliles}}, \binits{S.}},
\bauthor{\bsnm{{Carr}}, \binits{M.A.}},
\bauthor{\bsnm{{Castander}}, \binits{F.J.}},
\bauthor{\bsnm{{Cinabro}}, \binits{D.}},
\bauthor{\bsnm{{Connolly}}, \binits{A.J.}},
\bauthor{\bsnm{{Csabai}}, \binits{I.}},
\bauthor{\bsnm{{Cunha}}, \binits{C.E.}},
\bauthor{\bsnm{{Czarapata}}, \binits{P.C.}},
\bauthor{\bsnm{{Davenport}}, \binits{J.R.A.}},
\bauthor{\bsnm{{de Haas}}, \binits{E.}},
\bauthor{\bsnm{{Dilday}}, \binits{B.}},
\bauthor{\bsnm{{Doi}}, \binits{M.}},
\bauthor{\bsnm{{Eisenstein}}, \binits{D.J.}},
\bauthor{\bsnm{{Evans}}, \binits{M.L.}},
\bauthor{\bsnm{{Evans}}, \binits{N.W.}},
\bauthor{\bsnm{{Fan}}, \binits{X.}},
\bauthor{\bsnm{{Friedman}}, \binits{S.D.}},
\bauthor{\bsnm{{Frieman}}, \binits{J.A.}},
\bauthor{\bsnm{{Fukugita}}, \binits{M.}},
\bauthor{\bsnm{{G{\"a}nsicke}}, \binits{B.T.}},
\bauthor{\bsnm{{Gates}}, \binits{E.}},
\bauthor{\bsnm{{Gillespie}}, \binits{B.}},
\bauthor{\bsnm{{Gilmore}}, \binits{G.}},
\bauthor{\bsnm{{Gonzalez}}, \binits{B.}},
\bauthor{\bsnm{{Gonzalez}}, \binits{C.F.}},
\bauthor{\bsnm{{Grebel}}, \binits{E.K.}},
\bauthor{\bsnm{{Gunn}}, \binits{J.E.}},
\bauthor{\bsnm{{Gy{\"o}ry}}, \binits{Z.}},
\bauthor{\bsnm{{Hall}}, \binits{P.B.}},
\bauthor{\bsnm{{Harding}}, \binits{P.}},
\bauthor{\bsnm{{Harris}}, \binits{F.H.}},
\bauthor{\bsnm{{Harvanek}}, \binits{M.}},
\bauthor{\bsnm{{Hawley}}, \binits{S.L.}},
\bauthor{\bsnm{{Hayes}}, \binits{J.J.E.}},
\bauthor{\bsnm{{Heckman}}, \binits{T.M.}},
\bauthor{\bsnm{{Hendry}}, \binits{J.S.}},
\bauthor{\bsnm{{Hennessy}}, \binits{G.S.}},
\bauthor{\bsnm{{Hindsley}}, \binits{R.B.}},
\bauthor{\bsnm{{Hoblitt}}, \binits{J.}},
\bauthor{\bsnm{{Hogan}}, \binits{C.J.}},
\bauthor{\bsnm{{Hogg}}, \binits{D.W.}},
\bauthor{\bsnm{{Holtzman}}, \binits{J.A.}},
\bauthor{\bsnm{{Hyde}}, \binits{J.B.}},
\bauthor{\bsnm{{Ichikawa}}, \binits{S.-i.}},
\bauthor{\bsnm{{Ichikawa}}, \binits{T.}},
\bauthor{\bsnm{{Im}}, \binits{M.}},
\bauthor{\bsnm{{Ivezi{\'c}}}, \binits{{\v{Z}}.}},
\bauthor{\bsnm{{Jester}}, \binits{S.}},
\bauthor{\bsnm{{Jiang}}, \binits{L.}},
\bauthor{\bsnm{{Johnson}}, \binits{J.A.}},
\bauthor{\bsnm{{Jorgensen}}, \binits{A.M.}},
\bauthor{\bsnm{{Juri{\'c}}}, \binits{M.}},
\bauthor{\bsnm{{Kent}}, \binits{S.M.}},
\bauthor{\bsnm{{Kessler}}, \binits{R.}},
\bauthor{\bsnm{{Kleinman}}, \binits{S.J.}},
\bauthor{\bsnm{{Knapp}}, \binits{G.R.}},
\bauthor{\bsnm{{Konishi}}, \binits{K.}},
\bauthor{\bsnm{{Kron}}, \binits{R.G.}},
\bauthor{\bsnm{{Krzesinski}}, \binits{J.}},
\bauthor{\bsnm{{Kuropatkin}}, \binits{N.}},
\bauthor{\bsnm{{Lampeitl}}, \binits{H.}},
\bauthor{\bsnm{{Lebedeva}}, \binits{S.}},
\bauthor{\bsnm{{Lee}}, \binits{M.G.}},
\bauthor{\bsnm{{Lee}}, \binits{Y.S.}},
\bauthor{\bsnm{{French Leger}}, \binits{R.}},
\bauthor{\bsnm{{L{\'e}pine}}, \binits{S.}},
\bauthor{\bsnm{{Li}}, \binits{N.}},
\bauthor{\bsnm{{Lima}}, \binits{M.}},
\bauthor{\bsnm{{Lin}}, \binits{H.}},
\bauthor{\bsnm{{Long}}, \binits{D.C.}},
\bauthor{\bsnm{{Loomis}}, \binits{C.P.}},
\bauthor{\bsnm{{Loveday}}, \binits{J.}},
\bauthor{\bsnm{{Lupton}}, \binits{R.H.}},
\bauthor{\bsnm{{Magnier}}, \binits{E.}},
\bauthor{\bsnm{{Malanushenko}}, \binits{O.}},
\bauthor{\bsnm{{Malanushenko}}, \binits{V.}},
\bauthor{\bsnm{{Mandelbaum}}, \binits{R.}},
\bauthor{\bsnm{{Margon}}, \binits{B.}},
\bauthor{\bsnm{{Marriner}}, \binits{J.P.}},
\bauthor{\bsnm{{Mart{\'\i}nez-Delgado}}, \binits{D.}},
\bauthor{\bsnm{{Matsubara}}, \binits{T.}},
\bauthor{\bsnm{{McGehee}}, \binits{P.M.}},
\bauthor{\bsnm{{McKay}}, \binits{T.A.}},
\bauthor{\bsnm{{Meiksin}}, \binits{A.}},
\bauthor{\bsnm{{Morrison}}, \binits{H.L.}},
\bauthor{\bsnm{{Mullally}}, \binits{F.}},
\bauthor{\bsnm{{Munn}}, \binits{J.A.}},
\bauthor{\bsnm{{Murphy}}, \binits{T.}},
\bauthor{\bsnm{{Nash}}, \binits{T.}},
\bauthor{\bsnm{{Nebot}}, \binits{A.}},
\bauthor{\bsnm{{Neilsen}}, \binits{J.} \bsuffix{Eric~H.}},
\bauthor{\bsnm{{Newberg}}, \binits{H.J.}},
\bauthor{\bsnm{{Newman}}, \binits{P.R.}},
\bauthor{\bsnm{{Nichol}}, \binits{R.C.}},
\bauthor{\bsnm{{Nicinski}}, \binits{T.}},
\bauthor{\bsnm{{Nieto-Santisteban}}, \binits{M.}},
\bauthor{\bsnm{{Nitta}}, \binits{A.}},
\bauthor{\bsnm{{Okamura}}, \binits{S.}},
\bauthor{\bsnm{{Oravetz}}, \binits{D.J.}},
\bauthor{\bsnm{{Ostriker}}, \binits{J.P.}},
\bauthor{\bsnm{{Owen}}, \binits{R.}},
\bauthor{\bsnm{{Padmanabhan}}, \binits{N.}},
\bauthor{\bsnm{{Pan}}, \binits{K.}},
\bauthor{\bsnm{{Park}}, \binits{C.}},
\bauthor{\bsnm{{Pauls}}, \binits{G.}},
\bauthor{\bsnm{{Peoples}}, \binits{J.} \bsuffix{John}},
\bauthor{\bsnm{{Percival}}, \binits{W.J.}},
\bauthor{\bsnm{{Pier}}, \binits{J.R.}},
\bauthor{\bsnm{{Pope}}, \binits{A.C.}},
\bauthor{\bsnm{{Pourbaix}}, \binits{D.}},
\bauthor{\bsnm{{Price}}, \binits{P.A.}},
\bauthor{\bsnm{{Purger}}, \binits{N.}},
\bauthor{\bsnm{{Quinn}}, \binits{T.}},
\bauthor{\bsnm{{Raddick}}, \binits{M.J.}},
\bauthor{\bsnm{{Re Fiorentin}}, \binits{P.}},
\bauthor{\bsnm{{Richards}}, \binits{G.T.}},
\bauthor{\bsnm{{Richmond}}, \binits{M.W.}},
\bauthor{\bsnm{{Riess}}, \binits{A.G.}},
\bauthor{\bsnm{{Rix}}, \binits{H.-W.}},
\bauthor{\bsnm{{Rockosi}}, \binits{C.M.}},
\bauthor{\bsnm{{Sako}}, \binits{M.}},
\bauthor{\bsnm{{Schlegel}}, \binits{D.J.}},
\bauthor{\bsnm{{Schneider}}, \binits{D.P.}},
\bauthor{\bsnm{{Scholz}}, \binits{R.-D.}},
\bauthor{\bsnm{{Schreiber}}, \binits{M.R.}},
\bauthor{\bsnm{{Schwope}}, \binits{A.D.}},
\bauthor{\bsnm{{Seljak}}, \binits{U.}},
\bauthor{\bsnm{{Sesar}}, \binits{B.}},
\bauthor{\bsnm{{Sheldon}}, \binits{E.}},
\bauthor{\bsnm{{Shimasaku}}, \binits{K.}},
\bauthor{\bsnm{{Sibley}}, \binits{V.C.}},
\bauthor{\bsnm{{Simmons}}, \binits{A.E.}},
\bauthor{\bsnm{{Sivarani}}, \binits{T.}},
\bauthor{\bsnm{{Allyn Smith}}, \binits{J.}},
\bauthor{\bsnm{{Smith}}, \binits{M.C.}},
\bauthor{\bsnm{{Smol{\v{c}}i{\'c}}}, \binits{V.}},
\bauthor{\bsnm{{Snedden}}, \binits{S.A.}},
\bauthor{\bsnm{{Stebbins}}, \binits{A.}},
\bauthor{\bsnm{{Steinmetz}}, \binits{M.}},
\bauthor{\bsnm{{Stoughton}}, \binits{C.}},
\bauthor{\bsnm{{Strauss}}, \binits{M.A.}},
\bauthor{\bsnm{{SubbaRao}}, \binits{M.}},
\bauthor{\bsnm{{Suto}}, \binits{Y.}},
\bauthor{\bsnm{{Szalay}}, \binits{A.S.}},
\bauthor{\bsnm{{Szapudi}}, \binits{I.}},
\bauthor{\bsnm{{Szkody}}, \binits{P.}},
\bauthor{\bsnm{{Tanaka}}, \binits{M.}},
\bauthor{\bsnm{{Tegmark}}, \binits{M.}},
\bauthor{\bsnm{{Teodoro}}, \binits{L.F.A.}},
\bauthor{\bsnm{{Thakar}}, \binits{A.R.}},
\bauthor{\bsnm{{Tremonti}}, \binits{C.A.}},
\bauthor{\bsnm{{Tucker}}, \binits{D.L.}},
\bauthor{\bsnm{{Uomoto}}, \binits{A.}},
\bauthor{\bsnm{{Vanden Berk}}, \binits{D.E.}},
\bauthor{\bsnm{{Vandenberg}}, \binits{J.}},
\bauthor{\bsnm{{Vidrih}}, \binits{S.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
\bauthor{\bsnm{{Voges}}, \binits{W.}},
\bauthor{\bsnm{{Vogt}}, \binits{N.P.}},
\bauthor{\bsnm{{Wadadekar}}, \binits{Y.}},
\bauthor{\bsnm{{Watters}}, \binits{S.}},
\bauthor{\bsnm{{Weinberg}}, \binits{D.H.}},
\bauthor{\bsnm{{West}}, \binits{A.A.}},
\bauthor{\bsnm{{White}}, \binits{S.D.M.}},
\bauthor{\bsnm{{Wilhite}}, \binits{B.C.}},
\bauthor{\bsnm{{Wonders}}, \binits{A.C.}},
\bauthor{\bsnm{{Yanny}}, \binits{B.}},
\bauthor{\bsnm{{Yocum}}, \binits{D.R.}},
\bauthor{\bsnm{{York}}, \binits{D.G.}},
\bauthor{\bsnm{{Zehavi}}, \binits{I.}},
\bauthor{\bsnm{{Zibetti}}, \binits{S.}},
\end{comment}
\bauthor{et al.}:
\batitle{{The Seventh Data Release of the Sloan Digital Sky Survey}}.
\bjtitle{\apjs}
\bvolume{182}(\bissue{2}),
\bfpage{543}--\blpage{558}
(\byear{2009})
%{\href{https://arxiv.org/abs/0812.0649}{{arXiv:0812.0649}}}
%{[astro-ph]}.
%\doiurl{10.1088/0067-0049/182/2/543}
\end{barticle}
\endbibitem

%%% 22
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2017A&A...602A.100T}
\begin{barticle}
\bauthor{\bsnm{{Tempel}}, \binits{E.}},
\bauthor{\bsnm{{Tuvikene}}, \binits{T.}},
\bauthor{\bsnm{{Kipper}}, \binits{R.}},
\bauthor{\bsnm{{Libeskind}}, \binits{N.I.}}:
\batitle{{Merging groups and clusters of galaxies from the SDSS data. The
  catalogue of groups and potentially merging systems}}.
\bjtitle{\aap}
\bvolume{602},
\bfpage{100}
(\byear{2017})
%{\href{https://arxiv.org/abs/1704.04477}{{arXiv:1704.04477}}}
%{[astro-ph.CO]}.
%\doiurl{10.1051/0004-6361/201730499}
\end{barticle}
\endbibitem

%%% 23
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{1989ApJS...70....1A}
\begin{barticle}
\bauthor{\bsnm{{Abell}}, \binits{G.O.}},
\bauthor{\bsnm{{Corwin}}, \binits{J.} \bsuffix{Harold~G.}},
\bauthor{\bsnm{{Olowin}}, \binits{R.P.}}:
\batitle{{A Catalog of Rich Clusters of Galaxies}}.
\bjtitle{\apjs}
\bvolume{70},
\bfpage{1}
(\byear{1989}).
%\doiurl{10.1086/191333}
\end{barticle}
\endbibitem

%%% 24
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2002AJ....124.1810S}
\begin{barticle}
\bauthor{\bsnm{{Strauss}}, \binits{M.A.}},
\begin{comment}
\bauthor{\bsnm{{Weinberg}}, \binits{D.H.}},
\bauthor{\bsnm{{Lupton}}, \binits{R.H.}},
\bauthor{\bsnm{{Narayanan}}, \binits{V.K.}},
\bauthor{\bsnm{{Annis}}, \binits{J.}},
\bauthor{\bsnm{{Bernardi}}, \binits{M.}},
\bauthor{\bsnm{{Blanton}}, \binits{M.}},
\bauthor{\bsnm{{Burles}}, \binits{S.}},
\bauthor{\bsnm{{Connolly}}, \binits{A.J.}},
\bauthor{\bsnm{{Dalcanton}}, \binits{J.}},
\bauthor{\bsnm{{Doi}}, \binits{M.}},
\bauthor{\bsnm{{Eisenstein}}, \binits{D.}},
\bauthor{\bsnm{{Frieman}}, \binits{J.A.}},
\bauthor{\bsnm{{Fukugita}}, \binits{M.}},
\bauthor{\bsnm{{Gunn}}, \binits{J.E.}},
\bauthor{\bsnm{{Ivezi{\'c}}}, \binits{{\v{Z}}.}},
\bauthor{\bsnm{{Kent}}, \binits{S.}},
\bauthor{\bsnm{{Kim}}, \binits{R.S.J.}},
\bauthor{\bsnm{{Knapp}}, \binits{G.R.}},
\bauthor{\bsnm{{Kron}}, \binits{R.G.}},
\bauthor{\bsnm{{Munn}}, \binits{J.A.}},
\bauthor{\bsnm{{Newberg}}, \binits{H.J.}},
\bauthor{\bsnm{{Nichol}}, \binits{R.C.}},
\bauthor{\bsnm{{Okamura}}, \binits{S.}},
\bauthor{\bsnm{{Quinn}}, \binits{T.R.}},
\bauthor{\bsnm{{Richmond}}, \binits{M.W.}},
\bauthor{\bsnm{{Schlegel}}, \binits{D.J.}},
\bauthor{\bsnm{{Shimasaku}}, \binits{K.}},
\bauthor{\bsnm{{SubbaRao}}, \binits{M.}},
\bauthor{\bsnm{{Szalay}}, \binits{A.S.}},
\bauthor{\bsnm{{Vanden Berk}}, \binits{D.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}},
\bauthor{\bsnm{{Yanny}}, \binits{B.}},
\bauthor{\bsnm{{Yasuda}}, \binits{N.}},
\bauthor{\bsnm{{York}}, \binits{D.G.}},
\bauthor{\bsnm{{Zehavi}}, \binits{I.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Spectroscopic Target Selection in the Sloan Digital Sky Survey: The
  Main Galaxy Sample}}.
\bjtitle{\aj}
\bvolume{124}(\bissue{3}),
\bfpage{1810}--\blpage{1824}
(\byear{2002})
%{\href{https://arxiv.org/abs/astro-ph/0206225}{{arXiv:astro-ph/0206225}}}
%{[astro-ph]}.
%\doiurl{10.1086/342343}
\end{barticle}
\endbibitem

%%% 25
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2015A&A...578A.110A}
\begin{barticle}
\bauthor{\bsnm{{Argudo-Fern{\'a}ndez}}, \binits{M.}},
\begin{comment}
\bauthor{\bsnm{{Verley}}, \binits{S.}},
\bauthor{\bsnm{{Bergond}}, \binits{G.}},
\bauthor{\bsnm{{Duarte Puertas}}, \binits{S.}},
\bauthor{\bsnm{{Ramos Carmona}}, \binits{E.}},
\bauthor{\bsnm{{Sabater}}, \binits{J.}},
\bauthor{\bsnm{{Fern{\'a}ndez Lorenzo}}, \binits{M.}},
\bauthor{\bsnm{{Espada}}, \binits{D.}},
\bauthor{\bsnm{{Sulentic}}, \binits{J.}},
\bauthor{\bsnm{{Ruiz}}, \binits{J.E.}},
\bauthor{\bsnm{{Leon}}, \binits{S.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Catalogues of isolated galaxies, isolated pairs, and isolated
  triplets in the local Universe}}.
\bjtitle{\aap}
\bvolume{578},
\bfpage{110}
(\byear{2015})
%{\href{https://arxiv.org/abs/1504.00117}{{arXiv:1504.00117}}}
%{[astro-ph.GA]}.
%\doiurl{10.1051/0004-6361/201526016}
\end{barticle}
\endbibitem

%%% 26
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2006MNRAS.371..703S}
\begin{barticle}
\bauthor{\bsnm{{S{\'a}nchez-Bl{\'a}zquez}}, \binits{P.}},
\begin{comment}
\bauthor{\bsnm{{Peletier}}, \binits{R.F.}},
\bauthor{\bsnm{{Jim{\'e}nez-Vicente}}, \binits{J.}},
\bauthor{\bsnm{{Cardiel}}, \binits{N.}},
\bauthor{\bsnm{{Cenarro}}, \binits{A.J.}},
\bauthor{\bsnm{{Falc{\'o}n-Barroso}}, \binits{J.}},
\bauthor{\bsnm{{Gorgas}}, \binits{J.}},
\bauthor{\bsnm{{Selam}}, \binits{S.}},
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Medium-resolution Isaac Newton Telescope library of empirical
  spectra}}.
\bjtitle{\mnras}
\bvolume{371}(\bissue{2}),
\bfpage{703}--\blpage{718}
(\byear{2006})
%{\href{https://arxiv.org/abs/astro-ph/0607009}{{arXiv:astro-ph/0607009}}}
%{[astro-ph]}.
%\doiurl{10.1111/j.1365-2966.2006.10699.x}
\end{barticle}
\endbibitem

%%% 27
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2011A&A...532A..95F}
\begin{barticle}
\bauthor{\bsnm{{Falc{\'o}n-Barroso}}, \binits{J.}},
\begin{comment}
\bauthor{\bsnm{{S{\'a}nchez-Bl{\'a}zquez}}, \binits{P.}},
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}},
\bauthor{\bsnm{{Ricciardelli}}, \binits{E.}},
\bauthor{\bsnm{{Cardiel}}, \binits{N.}},
\bauthor{\bsnm{{Cenarro}}, \binits{A.J.}},
\bauthor{\bsnm{{Gorgas}}, \binits{J.}},
\bauthor{\bsnm{{Peletier}}, \binits{R.F.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{An updated MILES stellar library and stellar population models}}.
\bjtitle{\aap}
\bvolume{532},
\bfpage{95}
(\byear{2011})
%{\href{https://arxiv.org/abs/1107.2303}{{arXiv:1107.2303}}}
%{[astro-ph.CO]}.
%\doiurl{10.1051/0004-6361/201116842}
\end{barticle}
\endbibitem

%%% 28
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2015MNRAS.449.1177V}
\begin{barticle}
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}},
\begin{comment}
\bauthor{\bsnm{{Coelho}}, \binits{P.}},
\bauthor{\bsnm{{Cassisi}}, \binits{S.}},
\bauthor{\bsnm{{Ricciardelli}}, \binits{E.}},
\bauthor{\bsnm{{Falc{\'o}n-Barroso}}, \binits{J.}},
\bauthor{\bsnm{{S{\'a}nchez-Bl{\'a}zquez}}, \binits{P.}},
\bauthor{\bsnm{{La Barbera}}, \binits{F.}},
\bauthor{\bsnm{{Beasley}}, \binits{M.A.}},
\bauthor{\bsnm{{Pietrinferni}}, \binits{A.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Evolutionary stellar population synthesis with MILES - II.
  Scaled-solar and {\ensuremath{\alpha}}-enhanced models}}.
\bjtitle{\mnras}
\bvolume{449}(\bissue{2}),
\bfpage{1177}--\blpage{1214}
(\byear{2015})
%{\href{https://arxiv.org/abs/1504.08032}{{arXiv:1504.08032}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stv151}
\end{barticle}
\endbibitem

%%% 29
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2016MNRAS.463.3409V}
\begin{barticle}
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}},
\bauthor{\bsnm{{Koleva}}, \binits{M.}},
\bauthor{\bsnm{{Ricciardelli}}, \binits{E.}},
\bauthor{\bsnm{{R{\"o}ck}}, \binits{B.}},
\bauthor{\bsnm{{Falc{\'o}n-Barroso}}, \binits{J.}}:
\batitle{{UV-extended E-MILES stellar population models: young components in
  massive early-type galaxies}}.
\bjtitle{\mnras}
\bvolume{463}(\bissue{4}),
\bfpage{3409}--\blpage{3436}
(\byear{2016})
%{\href{https://arxiv.org/abs/1612.01187}{{arXiv:1612.01187}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stw2231}
\end{barticle}
\endbibitem

%%% 30
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2004PASP..116..138C}
\begin{barticle}
\bauthor{\bsnm{{Cappellari}}, \binits{M.}},
\bauthor{\bsnm{{Emsellem}}, \binits{E.}}:
\batitle{{Parametric Recovery of Line-of-Sight Velocity Distributions from
  Absorption-Line Spectra of Galaxies via Penalized Likelihood}}.
\bjtitle{\pasp}
\bvolume{116}(\bissue{816}),
\bfpage{138}--\blpage{147}
(\byear{2004})
%{\href{https://arxiv.org/abs/astro-ph/0312201}{{arXiv:astro-ph/0312201}}}
%{[astro-ph]}.
%\doiurl{10.1086/381875}
\end{barticle}
\endbibitem

%%% 31
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2017MNRAS.466..798C}
\begin{barticle}
\bauthor{\bsnm{{Cappellari}}, \binits{M.}}:
\batitle{{Improving the full spectrum fitting method: accurate convolution with
  Gauss-Hermite functions}}.
\bjtitle{\mnras}
\bvolume{466}(\bissue{1}),
\bfpage{798}--\blpage{811}
(\byear{2017})
%{\href{https://arxiv.org/abs/1607.08538}{{arXiv:1607.08538}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stw3020}
\end{barticle}
\endbibitem

%%% 32
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{Cappellari2022}
\begin{barticle}
\bauthor{\bsnm{{Cappellari}}, \binits{M.}}:
\batitle{{Full spectrum fitting with photometry in ppxf: non-parametric star
  formation history, metallicity and the quenching boundary from 3200 LEGA-C
  galaxies at redshift $z\approx0.8$}}.
\bjtitle{MNRAS submitted}
(\byear{2022})
%{\href{https://arxiv.org/abs/2208.14974}{{2208.14974}}}.
%\doiurl{10.48550/arXiv.2208.14974}
\end{barticle}
\endbibitem

%%% 33
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2006MNRAS.365...46O}
\begin{barticle}
\bauthor{\bsnm{{Ocvirk}}, \binits{P.}},
\bauthor{\bsnm{{Pichon}}, \binits{C.}},
\bauthor{\bsnm{{Lan{\c{c}}on}}, \binits{A.}},
\bauthor{\bsnm{{Thi{\'e}baut}}, \binits{E.}}:
\batitle{{STECMAP: STEllar Content from high-resolution galactic spectra via
  Maximum A Posteriori}}.
\bjtitle{\mnras}
\bvolume{365}(\bissue{1}),
\bfpage{46}--\blpage{73}
(\byear{2006})
%{\href{https://arxiv.org/abs/astro-ph/0505209}{{arXiv:astro-ph/0505209}}}
%{[astro-ph]}.
%\doiurl{10.1111/j.1365-2966.2005.09182.x}
\end{barticle}
\endbibitem

%%% 34
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2006MNRAS.365...74O}
\begin{barticle}
\bauthor{\bsnm{{Ocvirk}}, \binits{P.}},
\bauthor{\bsnm{{Pichon}}, \binits{C.}},
\bauthor{\bsnm{{Lan{\c{c}}on}}, \binits{A.}},
\bauthor{\bsnm{{Thi{\'e}baut}}, \binits{E.}}:
\batitle{{STECKMAP: STEllar Content and Kinematics from high resolution
  galactic spectra via Maximum A Posteriori}}.
\bjtitle{\mnras}
\bvolume{365}(\bissue{1}),
\bfpage{74}--\blpage{84}
(\byear{2006})
%{\href{https://arxiv.org/abs/astro-ph/0507002}{{arXiv:astro-ph/0507002}}}
%{[astro-ph]}.
%\doiurl{10.1111/j.1365-2966.2005.09323.x}
\end{barticle}
\endbibitem

%%% 35
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2004ApJ...612..168P}
\begin{barticle}
\bauthor{\bsnm{{Pietrinferni}}, \binits{A.}},
\bauthor{\bsnm{{Cassisi}}, \binits{S.}},
\bauthor{\bsnm{{Salaris}}, \binits{M.}},
\bauthor{\bsnm{{Castelli}}, \binits{F.}}:
\batitle{{A Large Stellar Evolution Database for Population Synthesis Studies.
  I. Scaled Solar Models and Isochrones}}.
\bjtitle{\apj}
\bvolume{612}(\bissue{1}),
\bfpage{168}--\blpage{190}
(\byear{2004})
%{\href{https://arxiv.org/abs/astro-ph/0405193}{{arXiv:astro-ph/0405193}}}
%{[astro-ph]}.
%\doiurl{10.1086/422498}
\end{barticle}
\endbibitem

%%% 36
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2001MNRAS.322..231K}
\begin{barticle}
\bauthor{\bsnm{{Kroupa}}, \binits{P.}}:
\batitle{{On the variation of the initial mass function}}.
\bjtitle{\mnras}
\bvolume{322}(\bissue{2}),
\bfpage{231}--\blpage{246}
(\byear{2001})
%{\href{https://arxiv.org/abs/astro-ph/0009005}{{arXiv:astro-ph/0009005}}}
%{[astro-ph]}.
%\doiurl{10.1046/j.1365-8711.2001.04022.x}
\end{barticle}
\endbibitem

%%% 37
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2019A&A...621A.120G}
\begin{barticle}
\bauthor{\bsnm{{Garc{\'\i}a-Benito}}, \binits{R.}},
\begin{comment}
\bauthor{\bsnm{{Gonz{\'a}lez Delgado}}, \binits{R.M.}},
\bauthor{\bsnm{{P{\'e}rez}}, \binits{E.}},
\bauthor{\bsnm{{Cid Fernandes}}, \binits{R.}},
\bauthor{\bsnm{{S{\'a}nchez}}, \binits{S.F.}},
\bauthor{\bsnm{{de Amorim}}, \binits{A.L.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Spatially resolved mass-to-light from the CALIFA survey.
  Mass-to-light ratio vs. color relations}}.
\bjtitle{\aap}
\bvolume{621},
\bfpage{120}
(\byear{2019})
%{\href{https://arxiv.org/abs/1811.08431}{{arXiv:1811.08431}}}
%{[astro-ph.GA]}.
%\doiurl{10.1051/0004-6361/201833993}
\end{barticle}
\endbibitem

%%% 38
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{MILESweb}
\begin{botherref}
MILES, Photometric Predictions.
\url{http://research.iac.es/proyecto/miles/pages/predicted-masses-and-photometric-observables-based-on-photometric-libraries.php}
\end{botherref}
\endbibitem

%%% 39
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{1996ApJS..106..307V}
\begin{barticle}
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}},
\bauthor{\bsnm{{Casuso}}, \binits{E.}},
\bauthor{\bsnm{{Peletier}}, \binits{R.F.}},
\bauthor{\bsnm{{Beckman}}, \binits{J.E.}}:
\batitle{{A New Chemo-evolutionary Population Synthesis Model for Early-Type
  Galaxies. I. Theoretical Basis}}.
\bjtitle{\apjs}
\bvolume{106},
\bfpage{307}
(\byear{1996})
%{\href{https://arxiv.org/abs/astro-ph/9605112}{{arXiv:astro-ph/9605112}}}
%{[astro-ph]}.
%\doiurl{10.1086/192340}
\end{barticle}
\endbibitem

%%% 40
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2001MNRAS.320..193B}
\begin{barticle}
\bauthor{\bsnm{{Blakeslee}}, \binits{J.P.}},
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}},
\bauthor{\bsnm{{Ajhar}}, \binits{E.A.}}:
\batitle{{Stellar populations and surface brightness fluctuations: new
  observations and models}}.
\bjtitle{\mnras}
\bvolume{320}(\bissue{2}),
\bfpage{193}--\blpage{216}
(\byear{2001})
%{\href{https://arxiv.org/abs/astro-ph/0008218}{{arXiv:astro-ph/0008218}}}
%{[astro-ph]}.
%\doiurl{10.1046/j.1365-8711.2001.03937.x}
\end{barticle}
\endbibitem

%%% 41
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2010MNRAS.404.1639V}
\begin{barticle}
\bauthor{\bsnm{{Vazdekis}}, \binits{A.}},
\begin{comment}
\bauthor{\bsnm{{S{\'a}nchez-Bl{\'a}zquez}}, \binits{P.}},
\bauthor{\bsnm{{Falc{\'o}n-Barroso}}, \binits{J.}},
\bauthor{\bsnm{{Cenarro}}, \binits{A.J.}},
\bauthor{\bsnm{{Beasley}}, \binits{M.A.}},
\bauthor{\bsnm{{Cardiel}}, \binits{N.}},
\bauthor{\bsnm{{Gorgas}}, \binits{J.}},
\bauthor{\bsnm{{Peletier}}, \binits{R.F.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Evolutionary stellar population synthesis with MILES - I. The base
  models and a new line index system}}.
\bjtitle{\mnras}
\bvolume{404}(\bissue{4}),
\bfpage{1639}--\blpage{1671}
(\byear{2010})
%{\href{https://arxiv.org/abs/1004.4439}{{arXiv:1004.4439}}}
%{[astro-ph.CO]}.
%\doiurl{10.1111/j.1365-2966.2010.16407.x}
\end{barticle}
\endbibitem

%%% 42
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2020A&A...638A..60A}
\begin{barticle}
\bauthor{\bsnm{{Alfaro}}, \binits{I.G.}},
\bauthor{\bsnm{{Rodriguez}}, \binits{F.}},
\bauthor{\bsnm{{Ruiz}}, \binits{A.N.}},
\bauthor{\bsnm{{Lambas}}, \binits{D.G.}}:
\batitle{{How galaxies populate haloes in very low-density environments. An
  analysis of the halo occupation distribution in cosmic voids}}.
\bjtitle{\aap}
\bvolume{638},
\bfpage{60}
(\byear{2020})
%{\href{https://arxiv.org/abs/2003.06255}{{arXiv:2003.06255}}}
%{[astro-ph.CO]}.
%\doiurl{10.1051/0004-6361/201937431}
\end{barticle}
\endbibitem

%%% 43
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2018MNRAS.480.3978A}
\begin{barticle}
\bauthor{\bsnm{{Artale}}, \binits{M.C.}},
\bauthor{\bsnm{{Zehavi}}, \binits{I.}},
\bauthor{\bsnm{{Contreras}}, \binits{S.}},
\bauthor{\bsnm{{Norberg}}, \binits{P.}}:
\batitle{{The impact of assembly bias on the halo occupation in hydrodynamical
  simulations}}.
\bjtitle{\mnras}
\bvolume{480}(\bissue{3}),
\bfpage{3978}--\blpage{3992}
(\byear{2018})
%{\href{https://arxiv.org/abs/1805.06938}{{arXiv:1805.06938}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/sty2110}
\end{barticle}
\endbibitem

%%% 44
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2020MNRAS.493..899H}
\begin{barticle}
\bauthor{\bsnm{{Habouzit}}, \binits{M.}},
\begin{comment}
\bauthor{\bsnm{{Pisani}}, \binits{A.}},
\bauthor{\bsnm{{Goulding}}, \binits{A.}},
\bauthor{\bsnm{{Dubois}}, \binits{Y.}},
\bauthor{\bsnm{{Somerville}}, \binits{R.S.}},
\bauthor{\bsnm{{Greene}}, \binits{J.E.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Properties of simulated galaxies and supermassive black holes in
  cosmic voids}}.
\bjtitle{\mnras}
\bvolume{493}(\bissue{1}),
\bfpage{899}--\blpage{921}
(\byear{2020})
%{\href{https://arxiv.org/abs/1912.06662}{{arXiv:1912.06662}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/staa219}
\end{barticle}
\endbibitem

%%% 45
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2022MNRAS.tmp.2385R}
\begin{barticle}
\bauthor{\bsnm{{Rosas-Guevara}}, \binits{Y.}},
\bauthor{\bsnm{{Tissera}}, \binits{P.}},
\bauthor{\bsnm{{Lagos}}, \binits{C.d.P.}},
\bauthor{\bsnm{{Paillas}}, \binits{E.}},
\bauthor{\bsnm{{Padilla}}, \binits{N.}}:
\batitle{{Revealing the properties of void galaxies and their assembly using
  the EAGLE simulation}}.
\bjtitle{\mnras}
(\byear{2022})
%{\href{https://arxiv.org/abs/2204.04565}{{arXiv:2204.04565}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stac2583}
\end{barticle}
\endbibitem

%%% 46
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2008ApJ...673..715C}
\begin{barticle}
\bauthor{\bsnm{{Constantin}}, \binits{A.}},
\bauthor{\bsnm{{Hoyle}}, \binits{F.}},
\bauthor{\bsnm{{Vogeley}}, \binits{M.S.}}:
\batitle{{Active Galactic Nuclei in Void Regions}}.
\bjtitle{\apj}
\bvolume{673}(\bissue{2}),
\bfpage{715}--\blpage{729}
(\byear{2008})
%{\href{https://arxiv.org/abs/0710.1631}{{arXiv:0710.1631}}}
%{[astro-ph]}.
%\doiurl{10.1086/524310}
\end{barticle}
\endbibitem

%%% 47
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2022MNRAS.509.1805C}
\begin{barticle}
\bauthor{\bsnm{{Ceccarelli}}, \binits{L.}},
\bauthor{\bsnm{{Duplancic}}, \binits{F.}},
\bauthor{\bsnm{{Garcia Lambas}}, \binits{D.}}:
\batitle{{The impact of void environment on AGN}}.
\bjtitle{\mnras}
\bvolume{509}(\bissue{2}),
\bfpage{1805}--\blpage{1819}
(\byear{2022}).
%\doiurl{10.1093/mnras/stab2902}
\end{barticle}
\endbibitem

%%% 48
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2019ApJ...874..140A}
\begin{barticle}
\bauthor{\bsnm{{Amiri}}, \binits{A.}},
\bauthor{\bsnm{{Tavasoli}}, \binits{S.}},
\bauthor{\bsnm{{De Zotti}}, \binits{G.}}:
\batitle{{Role of Environment on Nuclear Activity}}.
\bjtitle{\apj}
\bvolume{874}(\bissue{2}),
\bfpage{140}
(\byear{2019})
%{\href{https://arxiv.org/abs/1902.08757}{{arXiv:1902.08757}}}
%{[astro-ph.GA]}.
%\doiurl{10.3847/1538-4357/ab08e7}
\end{barticle}
\endbibitem

%%% 49
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2005MNRAS.363....2K}
\begin{barticle}
\bauthor{\bsnm{{Kere{\v{s}}}}, \binits{D.}},
\bauthor{\bsnm{{Katz}}, \binits{N.}},
\bauthor{\bsnm{{Weinberg}}, \binits{D.H.}},
\bauthor{\bsnm{{Dav{\'e}}}, \binits{R.}}:
\batitle{{How do galaxies get their gas?}}
\bjtitle{\mnras}
\bvolume{363}(\bissue{1}),
\bfpage{2}--\blpage{28}
(\byear{2005})
%{\href{https://arxiv.org/abs/astro-ph/0407095}{{arXiv:astro-ph/0407095}}}
%{[astro-ph]}.
%\doiurl{10.1111/j.1365-2966.2005.09451.x}
\end{barticle}
\endbibitem

%%% 50
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2022A&A...658A.124D}
\begin{barticle}
\bauthor{\bsnm{{Dom{\'\i}nguez-G{\'o}mez}}, \binits{J.}},
\begin{comment}
\bauthor{\bsnm{{Lisenfeld}}, \binits{U.}},
\bauthor{\bsnm{{P{\'e}rez}}, \binits{I.}},
\bauthor{\bsnm{{L{\'o}pez-S{\'a}nchez}}, \binits{{\'A}.R.}},
\bauthor{\bsnm{{Duarte Puertas}}, \binits{S.}},
\bauthor{\bsnm{{Falc{\'o}n-Barroso}}, \binits{J.}},
\bauthor{\bsnm{{Kreckel}}, \binits{K.}},
\bauthor{\bsnm{{Peletier}}, \binits{R.F.}},
\bauthor{\bsnm{{Ruiz-Lara}}, \binits{T.}},
\bauthor{\bsnm{{van de Weygaert}}, \binits{R.}},
\bauthor{\bsnm{{van der Hulst}}, \binits{J.M.}},
\bauthor{\bsnm{{Verley}}, \binits{S.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{CO-CAVITY pilot survey: Molecular gas and star formation in void
  galaxies}}.
\bjtitle{\aap}
\bvolume{658},
\bfpage{124}
(\byear{2022})
%{\href{https://arxiv.org/abs/2111.06844}{{arXiv:2111.06844}}}
%{[astro-ph.GA]}.
%\doiurl{10.1051/0004-6361/202141888}
\end{barticle}
\endbibitem

%%% 51
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{1986ApJ...301L..13K}
\begin{barticle}
\bauthor{\bsnm{{Kenney}}, \binits{J.D.}},
\bauthor{\bsnm{{Young}}, \binits{J.S.}}:
\batitle{{CO in H i--deficient Virgo Cluster Spiral Galaxies}}.
\bjtitle{\apjl}
\bvolume{301},
\bfpage{13}
(\byear{1986}).
%\doiurl{10.1086/184614}
\end{barticle}
\endbibitem

%%% 52
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{1997AJ....114.1753S}
\begin{barticle}
\bauthor{\bsnm{{Sage}}, \binits{L.J.}},
\bauthor{\bsnm{{Weistrop}}, \binits{D.}},
\bauthor{\bsnm{{Cruzen}}, \binits{S.}},
\bauthor{\bsnm{{Kompe}}, \binits{C.}}:
\batitle{{Molecular Gas and Star Formation Within Galaxies in the Bootes
  Void}}.
\bjtitle{\aj}
\bvolume{114},
\bfpage{1753}
(\byear{1997}).
%\doiurl{10.1086/118604}
\end{barticle}
\endbibitem

%%% 53
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2015ApJ...815...40D}
\begin{barticle}
\bauthor{\bsnm{{Das}}, \binits{M.}},
\bauthor{\bsnm{{Saito}}, \binits{T.}},
\bauthor{\bsnm{{Iono}}, \binits{D.}},
\bauthor{\bsnm{{Honey}}, \binits{M.}},
\bauthor{\bsnm{{Ramya}}, \binits{S.}}:
\batitle{{Detection of Molecular Gas in Void Galaxies : Implications for Star
  Formation in Isolated Environments}}.
\bjtitle{\apj}
\bvolume{815}(\bissue{1}),
\bfpage{40}
(\byear{2015})
%{\href{https://arxiv.org/abs/1510.07411}{{arXiv:1510.07411}}}
%{[astro-ph.GA]}.
%\doiurl{10.1088/0004-637X/815/1/40}
\end{barticle}
\endbibitem

%%% 54
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2016MNRAS.459.3574C}
\begin{barticle}
\bauthor{\bsnm{{Cortese}}, \binits{L.}},
\begin{comment}
\bauthor{\bsnm{{Bekki}}, \binits{K.}},
\bauthor{\bsnm{{Boselli}}, \binits{A.}},
\bauthor{\bsnm{{Catinella}}, \binits{B.}},
\bauthor{\bsnm{{Ciesla}}, \binits{L.}},
\bauthor{\bsnm{{Hughes}}, \binits{T.M.}},
\bauthor{\bsnm{{Baes}}, \binits{M.}},
\bauthor{\bsnm{{Bendo}}, \binits{G.J.}},
\bauthor{\bsnm{{Boquien}}, \binits{M.}},
\bauthor{\bsnm{{de Looze}}, \binits{I.}},
\bauthor{\bsnm{{Smith}}, \binits{M.W.L.}},
\bauthor{\bsnm{{Spinoglio}}, \binits{L.}},
\bauthor{\bsnm{{Viaene}}, \binits{S.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{The selective effect of environment on the atomic and molecular
  gas-to-dust ratio of nearby galaxies in the Herschel Reference Survey}}.
\bjtitle{\mnras}
\bvolume{459}(\bissue{4}),
\bfpage{3574}--\blpage{3584}
(\byear{2016})
%{\href{https://arxiv.org/abs/1604.01505}{{arXiv:1604.01505}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/stw801}
\end{barticle}
\endbibitem

%%% 55
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2016A&A...590A..27G}
\begin{barticle}
\bauthor{\bsnm{{Grossi}}, \binits{M.}},
\begin{comment}
\bauthor{\bsnm{{Corbelli}}, \binits{E.}},
\bauthor{\bsnm{{Bizzocchi}}, \binits{L.}},
\bauthor{\bsnm{{Giovanardi}}, \binits{C.}},
\bauthor{\bsnm{{Bomans}}, \binits{D.}},
\bauthor{\bsnm{{Coelho}}, \binits{B.}},
\bauthor{\bsnm{{De Looze}}, \binits{I.}},
\bauthor{\bsnm{{Gon{\c{c}}alves}}, \binits{T.S.}},
\bauthor{\bsnm{{Hunt}}, \binits{L.K.}},
\bauthor{\bsnm{{Leonardo}}, \binits{E.}},
\bauthor{\bsnm{{Madden}}, \binits{S.}},
\bauthor{\bsnm{{Men{\'e}ndez-Delmestre}}, \binits{K.}},
\bauthor{\bsnm{{Pappalardo}}, \binits{C.}},
\bauthor{\bsnm{{Riguccini}}, \binits{L.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{Star-forming dwarf galaxies in the Virgo cluster: the link between
  molecular gas, atomic gas, and dust}}.
\bjtitle{\aap}
\bvolume{590},
\bfpage{27}
(\byear{2016})
%{\href{https://arxiv.org/abs/1602.09077}{{arXiv:1602.09077}}}
%{[astro-ph.GA]}.
%\doiurl{10.1051/0004-6361/201628123}
\end{barticle}
\endbibitem

%%% 56
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2020ApJS..249....3A}
\begin{barticle}
\bauthor{\bsnm{{Ahumada}}, \binits{R.}},
\begin{comment}
\bauthor{\bsnm{{Prieto}}, \binits{C.A.}},
\bauthor{\bsnm{{Almeida}}, \binits{A.}},
\bauthor{\bsnm{{Anders}}, \binits{F.}},
\bauthor{\bsnm{{Anderson}}, \binits{S.F.}},
\bauthor{\bsnm{{Andrews}}, \binits{B.H.}},
\bauthor{\bsnm{{Anguiano}}, \binits{B.}},
\bauthor{\bsnm{{Arcodia}}, \binits{R.}},
\bauthor{\bsnm{{Armengaud}}, \binits{E.}},
\bauthor{\bsnm{{Aubert}}, \binits{M.}},
\bauthor{\bsnm{{Avila}}, \binits{S.}},
\bauthor{\bsnm{{Avila-Reese}}, \binits{V.}},
\bauthor{\bsnm{{Badenes}}, \binits{C.}},
\bauthor{\bsnm{{Balland}}, \binits{C.}},
\bauthor{\bsnm{{Barger}}, \binits{K.}},
\bauthor{\bsnm{{Barrera-Ballesteros}}, \binits{J.K.}},
\bauthor{\bsnm{{Basu}}, \binits{S.}},
\bauthor{\bsnm{{Bautista}}, \binits{J.}},
\bauthor{\bsnm{{Beaton}}, \binits{R.L.}},
\bauthor{\bsnm{{Beers}}, \binits{T.C.}},
\bauthor{\bsnm{{Benavides}}, \binits{B.I.T.}},
\bauthor{\bsnm{{Bender}}, \binits{C.F.}},
\bauthor{\bsnm{{Bernardi}}, \binits{M.}},
\bauthor{\bsnm{{Bershady}}, \binits{M.}},
\bauthor{\bsnm{{Beutler}}, \binits{F.}},
\bauthor{\bsnm{{Bidin}}, \binits{C.M.}},
\bauthor{\bsnm{{Bird}}, \binits{J.}},
\bauthor{\bsnm{{Bizyaev}}, \binits{D.}},
\bauthor{\bsnm{{Blanc}}, \binits{G.A.}},
\bauthor{\bsnm{{Blanton}}, \binits{M.R.}},
\bauthor{\bsnm{{Boquien}}, \binits{M.}},
\bauthor{\bsnm{{Borissova}}, \binits{J.}},
\bauthor{\bsnm{{Bovy}}, \binits{J.}},
\bauthor{\bsnm{{Brandt}}, \binits{W.N.}},
\bauthor{\bsnm{{Brinkmann}}, \binits{J.}},
\bauthor{\bsnm{{Brownstein}}, \binits{J.R.}},
\bauthor{\bsnm{{Bundy}}, \binits{K.}},
\bauthor{\bsnm{{Bureau}}, \binits{M.}},
\bauthor{\bsnm{{Burgasser}}, \binits{A.}},
\bauthor{\bsnm{{Burtin}}, \binits{E.}},
\bauthor{\bsnm{{Cano-D{\'\i}az}}, \binits{M.}},
\bauthor{\bsnm{{Capasso}}, \binits{R.}},
\bauthor{\bsnm{{Cappellari}}, \binits{M.}},
\bauthor{\bsnm{{Carrera}}, \binits{R.}},
\bauthor{\bsnm{{Chabanier}}, \binits{S.}},
\bauthor{\bsnm{{Chaplin}}, \binits{W.}},
\bauthor{\bsnm{{Chapman}}, \binits{M.}},
\bauthor{\bsnm{{Cherinka}}, \binits{B.}},
\bauthor{\bsnm{{Chiappini}}, \binits{C.}},
\bauthor{\bsnm{{Doohyun Choi}}, \binits{P.}},
\bauthor{\bsnm{{Chojnowski}}, \binits{S.D.}},
\bauthor{\bsnm{{Chung}}, \binits{H.}},
\bauthor{\bsnm{{Clerc}}, \binits{N.}},
\bauthor{\bsnm{{Coffey}}, \binits{D.}},
\bauthor{\bsnm{{Comerford}}, \binits{J.M.}},
\bauthor{\bsnm{{Comparat}}, \binits{J.}},
\bauthor{\bsnm{{da Costa}}, \binits{L.}},
\bauthor{\bsnm{{Cousinou}}, \binits{M.-C.}},
\bauthor{\bsnm{{Covey}}, \binits{K.}},
\bauthor{\bsnm{{Crane}}, \binits{J.D.}},
\bauthor{\bsnm{{Cunha}}, \binits{K.}},
\bauthor{\bsnm{{Ilha}}, \binits{G.d.S.}},
\bauthor{\bsnm{{Dai}}, \binits{Y.S.}},
\bauthor{\bsnm{{Damsted}}, \binits{S.B.}},
\bauthor{\bsnm{{Darling}}, \binits{J.}},
\bauthor{\bsnm{{Davidson}}, \binits{J.} \bsuffix{James~W.}},
\bauthor{\bsnm{{Davies}}, \binits{R.}},
\bauthor{\bsnm{{Dawson}}, \binits{K.}},
\bauthor{\bsnm{{De}}, \binits{N.}},
\bauthor{\bsnm{{de la Macorra}}, \binits{A.}},
\bauthor{\bsnm{{De Lee}}, \binits{N.}},
\bauthor{\bsnm{{Queiroz}}, \binits{A.B.d.A.}},
\bauthor{\bsnm{{Deconto Machado}}, \binits{A.}},
\bauthor{\bsnm{{de la Torre}}, \binits{S.}},
\bauthor{\bsnm{{Dell'Agli}}, \binits{F.}},
\bauthor{\bsnm{{du Mas des Bourboux}}, \binits{H.}},
\bauthor{\bsnm{{Diamond-Stanic}}, \binits{A.M.}},
\bauthor{\bsnm{{Dillon}}, \binits{S.}},
\bauthor{\bsnm{{Donor}}, \binits{J.}},
\bauthor{\bsnm{{Drory}}, \binits{N.}},
\bauthor{\bsnm{{Duckworth}}, \binits{C.}},
\bauthor{\bsnm{{Dwelly}}, \binits{T.}},
\bauthor{\bsnm{{Ebelke}}, \binits{G.}},
\bauthor{\bsnm{{Eftekharzadeh}}, \binits{S.}},
\bauthor{\bsnm{{Davis Eigenbrot}}, \binits{A.}},
\bauthor{\bsnm{{Elsworth}}, \binits{Y.P.}},
\bauthor{\bsnm{{Eracleous}}, \binits{M.}},
\bauthor{\bsnm{{Erfanianfar}}, \binits{G.}},
\bauthor{\bsnm{{Escoffier}}, \binits{S.}},
\bauthor{\bsnm{{Fan}}, \binits{X.}},
\bauthor{\bsnm{{Farr}}, \binits{E.}},
\bauthor{\bsnm{{Fern{\'a}ndez-Trincado}}, \binits{J.G.}},
\bauthor{\bsnm{{Feuillet}}, \binits{D.}},
\bauthor{\bsnm{{Finoguenov}}, \binits{A.}},
\bauthor{\bsnm{{Fofie}}, \binits{P.}},
\bauthor{\bsnm{{Fraser-McKelvie}}, \binits{A.}},
\bauthor{\bsnm{{Frinchaboy}}, \binits{P.M.}},
\bauthor{\bsnm{{Fromenteau}}, \binits{S.}},
\bauthor{\bsnm{{Fu}}, \binits{H.}},
\bauthor{\bsnm{{Galbany}}, \binits{L.}},
\bauthor{\bsnm{{Garcia}}, \binits{R.A.}},
\bauthor{\bsnm{{Garc{\'\i}a-Hern{\'a}ndez}}, \binits{D.A.}},
\bauthor{\bsnm{{Oehmichen}}, \binits{L.A.G.}},
\bauthor{\bsnm{{Ge}}, \binits{J.}},
\bauthor{\bsnm{{Maia}}, \binits{M.A.G.}},
\bauthor{\bsnm{{Geisler}}, \binits{D.}},
\bauthor{\bsnm{{Gelfand}}, \binits{J.}},
\bauthor{\bsnm{{Goddy}}, \binits{J.}},
\bauthor{\bsnm{{Gonzalez-Perez}}, \binits{V.}},
\bauthor{\bsnm{{Grabowski}}, \binits{K.}},
\bauthor{\bsnm{{Green}}, \binits{P.}},
\bauthor{\bsnm{{Grier}}, \binits{C.J.}},
\bauthor{\bsnm{{Guo}}, \binits{H.}},
\bauthor{\bsnm{{Guy}}, \binits{J.}},
\bauthor{\bsnm{{Harding}}, \binits{P.}},
\bauthor{\bsnm{{Hasselquist}}, \binits{S.}},
\bauthor{\bsnm{{Hawken}}, \binits{A.J.}},
\bauthor{\bsnm{{Hayes}}, \binits{C.R.}},
\bauthor{\bsnm{{Hearty}}, \binits{F.}},
\bauthor{\bsnm{{Hekker}}, \binits{S.}},
\bauthor{\bsnm{{Hogg}}, \binits{D.W.}},
\bauthor{\bsnm{{Holtzman}}, \binits{J.A.}},
\bauthor{\bsnm{{Horta}}, \binits{D.}},
\bauthor{\bsnm{{Hou}}, \binits{J.}},
\bauthor{\bsnm{{Hsieh}}, \binits{B.-C.}},
\bauthor{\bsnm{{Huber}}, \binits{D.}},
\bauthor{\bsnm{{Hunt}}, \binits{J.A.S.}},
\bauthor{\bsnm{{Chitham}}, \binits{J.I.}},
\bauthor{\bsnm{{Imig}}, \binits{J.}},
\bauthor{\bsnm{{Jaber}}, \binits{M.}},
\bauthor{\bsnm{{Angel}}, \binits{C.E.J.}},
\bauthor{\bsnm{{Johnson}}, \binits{J.A.}},
\bauthor{\bsnm{{Jones}}, \binits{A.M.}},
\bauthor{\bsnm{{J{\"o}nsson}}, \binits{H.}},
\bauthor{\bsnm{{Jullo}}, \binits{E.}},
\bauthor{\bsnm{{Kim}}, \binits{Y.}},
\bauthor{\bsnm{{Kinemuchi}}, \binits{K.}},
\bauthor{\bsnm{{Kirkpatrick}}, \binits{I.} \bsuffix{Charles~C.}},
\bauthor{\bsnm{{Kite}}, \binits{G.W.}},
\bauthor{\bsnm{{Klaene}}, \binits{M.}},
\bauthor{\bsnm{{Kneib}}, \binits{J.-P.}},
\bauthor{\bsnm{{Kollmeier}}, \binits{J.A.}},
\bauthor{\bsnm{{Kong}}, \binits{H.}},
\bauthor{\bsnm{{Kounkel}}, \binits{M.}},
\bauthor{\bsnm{{Krishnarao}}, \binits{D.}},
\bauthor{\bsnm{{Lacerna}}, \binits{I.}},
\bauthor{\bsnm{{Lan}}, \binits{T.-W.}},
\bauthor{\bsnm{{Lane}}, \binits{R.R.}},
\bauthor{\bsnm{{Law}}, \binits{D.R.}},
\bauthor{\bsnm{{Le Goff}}, \binits{J.-M.}},
\bauthor{\bsnm{{Leung}}, \binits{H.W.}},
\bauthor{\bsnm{{Lewis}}, \binits{H.}},
\bauthor{\bsnm{{Li}}, \binits{C.}},
\bauthor{\bsnm{{Lian}}, \binits{J.}},
\bauthor{\bsnm{{Lin}}, \binits{L.}},
\bauthor{\bsnm{{Long}}, \binits{D.}},
\bauthor{\bsnm{{Longa-Pe{\~n}a}}, \binits{P.}},
\bauthor{\bsnm{{Lundgren}}, \binits{B.}},
\bauthor{\bsnm{{Lyke}}, \binits{B.W.}},
\bauthor{\bsnm{{Ted Mackereth}}, \binits{J.}},
\bauthor{\bsnm{{MacLeod}}, \binits{C.L.}},
\bauthor{\bsnm{{Majewski}}, \binits{S.R.}},
\bauthor{\bsnm{{Manchado}}, \binits{A.}},
\bauthor{\bsnm{{Maraston}}, \binits{C.}},
\bauthor{\bsnm{{Martini}}, \binits{P.}},
\bauthor{\bsnm{{Masseron}}, \binits{T.}},
\bauthor{\bsnm{{Masters}}, \binits{K.L.}},
\bauthor{\bsnm{{Mathur}}, \binits{S.}},
\bauthor{\bsnm{{McDermid}}, \binits{R.M.}},
\bauthor{\bsnm{{Merloni}}, \binits{A.}},
\bauthor{\bsnm{{Merrifield}}, \binits{M.}},
\bauthor{\bsnm{{M{\'e}sz{\'a}ros}}, \binits{S.}},
\bauthor{\bsnm{{Miglio}}, \binits{A.}},
\bauthor{\bsnm{{Minniti}}, \binits{D.}},
\bauthor{\bsnm{{Minsley}}, \binits{R.}},
\bauthor{\bsnm{{Miyaji}}, \binits{T.}},
\bauthor{\bsnm{{Mohammad}}, \binits{F.G.}},
\bauthor{\bsnm{{Mosser}}, \binits{B.}},
\bauthor{\bsnm{{Mueller}}, \binits{E.-M.}},
\bauthor{\bsnm{{Muna}}, \binits{D.}},
\bauthor{\bsnm{{Mu{\~n}oz-Guti{\'e}rrez}}, \binits{A.}},
\bauthor{\bsnm{{Myers}}, \binits{A.D.}},
\bauthor{\bsnm{{Nadathur}}, \binits{S.}},
\bauthor{\bsnm{{Nair}}, \binits{P.}},
\bauthor{\bsnm{{Nandra}}, \binits{K.}},
\bauthor{\bsnm{{do Nascimento}}, \binits{J.C.}},
\bauthor{\bsnm{{Nevin}}, \binits{R.J.}},
\bauthor{\bsnm{{Newman}}, \binits{J.A.}},
\bauthor{\bsnm{{Nidever}}, \binits{D.L.}},
\bauthor{\bsnm{{Nitschelm}}, \binits{C.}},
\bauthor{\bsnm{{Noterdaeme}}, \binits{P.}},
\bauthor{\bsnm{{O'Connell}}, \binits{J.E.}},
\bauthor{\bsnm{{Olmstead}}, \binits{M.D.}},
\bauthor{\bsnm{{Oravetz}}, \binits{D.}},
\bauthor{\bsnm{{Oravetz}}, \binits{A.}},
\bauthor{\bsnm{{Osorio}}, \binits{Y.}},
\bauthor{\bsnm{{Pace}}, \binits{Z.J.}},
\bauthor{\bsnm{{Padilla}}, \binits{N.}},
\bauthor{\bsnm{{Palanque-Delabrouille}}, \binits{N.}},
\bauthor{\bsnm{{Palicio}}, \binits{P.A.}},
\bauthor{\bsnm{{Pan}}, \binits{H.-A.}},
\bauthor{\bsnm{{Pan}}, \binits{K.}},
\bauthor{\bsnm{{Parker}}, \binits{J.}},
\bauthor{\bsnm{{Paviot}}, \binits{R.}},
\bauthor{\bsnm{{Peirani}}, \binits{S.}},
\bauthor{\bsnm{{Ram{\'r}ez}}, \binits{K.P.}},
\bauthor{\bsnm{{Penny}}, \binits{S.}},
\bauthor{\bsnm{{Percival}}, \binits{W.J.}},
\bauthor{\bsnm{{Perez-Fournon}}, \binits{I.}},
\bauthor{\bsnm{{P{\'e}rez-R{\`a}fols}}, \binits{I.}},
\bauthor{\bsnm{{Petitjean}}, \binits{P.}},
\bauthor{\bsnm{{Pieri}}, \binits{M.M.}},
\bauthor{\bsnm{{Pinsonneault}}, \binits{M.}},
\bauthor{\bsnm{{Poovelil}}, \binits{V.J.}},
\bauthor{\bsnm{{Povick}}, \binits{J.T.}},
\bauthor{\bsnm{{Prakash}}, \binits{A.}},
\bauthor{\bsnm{{Price-Whelan}}, \binits{A.M.}},
\bauthor{\bsnm{{Raddick}}, \binits{M.J.}},
\bauthor{\bsnm{{Raichoor}}, \binits{A.}},
\bauthor{\bsnm{{Ray}}, \binits{A.}},
\bauthor{\bsnm{{Rembold}}, \binits{S.B.}},
\bauthor{\bsnm{{Rezaie}}, \binits{M.}},
\bauthor{\bsnm{{Riffel}}, \binits{R.A.}},
\bauthor{\bsnm{{Riffel}}, \binits{R.}},
\bauthor{\bsnm{{Rix}}, \binits{H.-W.}},
\bauthor{\bsnm{{Robin}}, \binits{A.C.}},
\bauthor{\bsnm{{Roman-Lopes}}, \binits{A.}},
\bauthor{\bsnm{{Rom{\'a}n-Z{\'u}{\~n}iga}}, \binits{C.}},
\bauthor{\bsnm{{Rose}}, \binits{B.}},
\bauthor{\bsnm{{Ross}}, \binits{A.J.}},
\bauthor{\bsnm{{Rossi}}, \binits{G.}},
\bauthor{\bsnm{{Rowlands}}, \binits{K.}},
\bauthor{\bsnm{{Rubin}}, \binits{K.H.R.}},
\bauthor{\bsnm{{Salvato}}, \binits{M.}},
\bauthor{\bsnm{{S{\'a}nchez}}, \binits{A.G.}},
\bauthor{\bsnm{{S{\'a}nchez-Menguiano}}, \binits{L.}},
\bauthor{\bsnm{{S{\'a}nchez-Gallego}}, \binits{J.R.}},
\bauthor{\bsnm{{Sayres}}, \binits{C.}},
\bauthor{\bsnm{{Schaefer}}, \binits{A.}},
\bauthor{\bsnm{{Schiavon}}, \binits{R.P.}},
\bauthor{\bsnm{{Schimoia}}, \binits{J.S.}},
\bauthor{\bsnm{{Schlafly}}, \binits{E.}},
\bauthor{\bsnm{{Schlegel}}, \binits{D.}},
\bauthor{\bsnm{{Schneider}}, \binits{D.P.}},
\bauthor{\bsnm{{Schultheis}}, \binits{M.}},
\bauthor{\bsnm{{Schwope}}, \binits{A.}},
\bauthor{\bsnm{{Seo}}, \binits{H.-J.}},
\bauthor{\bsnm{{Serenelli}}, \binits{A.}},
\bauthor{\bsnm{{Shafieloo}}, \binits{A.}},
\bauthor{\bsnm{{Shamsi}}, \binits{S.J.}},
\bauthor{\bsnm{{Shao}}, \binits{Z.}},
\bauthor{\bsnm{{Shen}}, \binits{S.}},
\bauthor{\bsnm{{Shetrone}}, \binits{M.}},
\bauthor{\bsnm{{Shirley}}, \binits{R.}},
\bauthor{\bsnm{{Aguirre}}, \binits{V.S.}},
\bauthor{\bsnm{{Simon}}, \binits{J.D.}},
\bauthor{\bsnm{{Skrutskie}}, \binits{M.F.}},
\bauthor{\bsnm{{Slosar}}, \binits{A.}},
\bauthor{\bsnm{{Smethurst}}, \binits{R.}},
\bauthor{\bsnm{{Sobeck}}, \binits{J.}},
\bauthor{\bsnm{{Sodi}}, \binits{B.C.}},
\bauthor{\bsnm{{Souto}}, \binits{D.}},
\bauthor{\bsnm{{Stark}}, \binits{D.V.}},
\bauthor{\bsnm{{Stassun}}, \binits{K.G.}},
\bauthor{\bsnm{{Steinmetz}}, \binits{M.}},
\bauthor{\bsnm{{Stello}}, \binits{D.}},
\bauthor{\bsnm{{Stermer}}, \binits{J.}},
\bauthor{\bsnm{{Storchi-Bergmann}}, \binits{T.}},
\bauthor{\bsnm{{Streblyanska}}, \binits{A.}},
\bauthor{\bsnm{{Stringfellow}}, \binits{G.S.}},
\bauthor{\bsnm{{Stutz}}, \binits{A.}},
\bauthor{\bsnm{{Su{\'a}rez}}, \binits{G.}},
\bauthor{\bsnm{{Sun}}, \binits{J.}},
\bauthor{\bsnm{{Taghizadeh-Popp}}, \binits{M.}},
\bauthor{\bsnm{{Talbot}}, \binits{M.S.}},
\bauthor{\bsnm{{Tayar}}, \binits{J.}},
\bauthor{\bsnm{{Thakar}}, \binits{A.R.}},
\bauthor{\bsnm{{Theriault}}, \binits{R.}},
\bauthor{\bsnm{{Thomas}}, \binits{D.}},
\bauthor{\bsnm{{Thomas}}, \binits{Z.C.}},
\bauthor{\bsnm{{Tinker}}, \binits{J.}},
\bauthor{\bsnm{{Tojeiro}}, \binits{R.}},
\bauthor{\bsnm{{Toledo}}, \binits{H.H.}},
\bauthor{\bsnm{{Tremonti}}, \binits{C.A.}},
\bauthor{\bsnm{{Troup}}, \binits{N.W.}},
\bauthor{\bsnm{{Tuttle}}, \binits{S.}},
\bauthor{\bsnm{{Unda-Sanzana}}, \binits{E.}},
\bauthor{\bsnm{{Valentini}}, \binits{M.}},
\bauthor{\bsnm{{Vargas-Gonz{\'a}lez}}, \binits{J.}},
\bauthor{\bsnm{{Vargas-Maga{\~n}a}}, \binits{M.}},
\bauthor{\bsnm{{V{\'a}zquez-Mata}}, \binits{J.A.}},
\bauthor{\bsnm{{Vivek}}, \binits{M.}},
\bauthor{\bsnm{{Wake}}, \binits{D.}},
\bauthor{\bsnm{{Wang}}, \binits{Y.}},
\bauthor{\bsnm{{Weaver}}, \binits{B.A.}},
\bauthor{\bsnm{{Weijmans}}, \binits{A.-M.}},
\bauthor{\bsnm{{Wild}}, \binits{V.}},
\bauthor{\bsnm{{Wilson}}, \binits{J.C.}},
\bauthor{\bsnm{{Wilson}}, \binits{R.F.}},
\bauthor{\bsnm{{Wolthuis}}, \binits{N.}},
\bauthor{\bsnm{{Wood-Vasey}}, \binits{W.M.}},
\bauthor{\bsnm{{Yan}}, \binits{R.}},
\bauthor{\bsnm{{Yang}}, \binits{M.}},
\bauthor{\bsnm{{Y{\`e}che}}, \binits{C.}},
\bauthor{\bsnm{{Zamora}}, \binits{O.}},
\bauthor{\bsnm{{Zarrouk}}, \binits{P.}},
\bauthor{\bsnm{{Zasowski}}, \binits{G.}},
\bauthor{\bsnm{{Zhang}}, \binits{K.}},
\bauthor{\bsnm{{Zhao}}, \binits{C.}},
\bauthor{\bsnm{{Zhao}}, \binits{G.}},
\bauthor{\bsnm{{Zheng}}, \binits{Z.}},
\bauthor{\bsnm{{Zheng}}, \binits{Z.}},
\bauthor{\bsnm{{Zhu}}, \binits{G.}},
\bauthor{\bsnm{{Zou}}, \binits{H.}}:
\end{comment}
\bauthor{et al.}:
\batitle{{The 16th Data Release of the Sloan Digital Sky Surveys: First Release
  from the APOGEE-2 Southern Survey and Full Release of eBOSS Spectra}}.
\bjtitle{\apjs}
\bvolume{249}(\bissue{1}),
\bfpage{3}
(\byear{2020})
%{\href{https://arxiv.org/abs/1912.02905}{{arXiv:1912.02905}}}
%{[astro-ph.GA]}.
%\doiurl{10.3847/1538-4365/ab929e}
\end{barticle}
\endbibitem

%%% 57
\stepcounter{mycounterbib}\bibitem[\themycounterbib]{2018MNRAS.476.3661D}
\begin{barticle}
\bauthor{\bsnm{{Dom{\'\i}nguez S{\'a}nchez}}, \binits{H.}},
\bauthor{\bsnm{{Huertas-Company}}, \binits{M.}},
\bauthor{\bsnm{{Bernardi}}, \binits{M.}},
\bauthor{\bsnm{{Tuccillo}}, \binits{D.}},
\bauthor{\bsnm{{Fischer}}, \binits{J.L.}}:
\batitle{{Improving galaxy morphologies for SDSS with Deep Learning}}.
\bjtitle{\mnras}
\bvolume{476}(\bissue{3}),
\bfpage{3661}--\blpage{3676}
(\byear{2018})
%{\href{https://arxiv.org/abs/1711.05744}{{arXiv:1711.05744}}}
%{[astro-ph.GA]}.
%\doiurl{10.1093/mnras/sty338}
\end{barticle}
\endbibitem

\end{thebibliography}

